A framework for constrained static state estimation in unbalanced distribution networks

State estimation plays a key role in the transition from the passive to the active operation of distribution systems, as it allows to monitor these networks and, successively, to perform control actions. However, designing state estimators for distribution systems carries a significant amount of challenges. This is due to the physical complexity of the networks, e.g., phase unbalance, and limited measurements. Furthermore, the features of the distribution system present significant local variations, e.g., voltage level and number and type of customers, which makes it hard to design a "one-size-fits-all" state estimator. The present paper introduces a unifying framework that allows to easily implement and compare diverse unbalanced static state estimation models. This is achieved by formulating state estimation as a general constrained optimization problem. The advantages of this approach are described and supported by numerical illustration on a large set of distribution feeders. The framework is also implemented and made available open-source.

==> sections/0_Nomenclature.tex <==
The sets, parameters and variables that are used throughout the paper are here introduced. Power lines are represented as a $\pi$ model, as illustrated in Fig. \ref{fig:line}. Bold letters indicate matrices and vectors. 

\addcontentsline{toc}{section}{Nomenclature}
%%%%%%%%%%%%
\subsection*{Sets}
%%%%%%%%%%%%
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{xxxxxxxxxx}]
    \item[\buses] Feeder buses
	\item[\branches, \branchesi] Feeder branches, branches from/to bus $i$
	\item[\gens, \gensi] Feeder generators, generators at bus $i$
	\item[\loads, \loadsi] Feeder loads, loads at bus $i$
	\item[\meas] Measurements
	\item[\shuntsi] Shunt elements at bus $i$
	\item[\rbuses] Reference buses
    \item[\conds, \condsij] Conductors, conductors of branch $(i,j)$
 \end{IEEEdescription} \vspace{-0.3cm} 
\subsection*{Line variables and parameters} 
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{xxxxxxxxxxx}]
	\item[$\mathbf{U}_i := {[U_{i,c}]_{\phi \in \Phi}}$] Complex voltage of bus $i$ 
	\item[$\mathbf{Z}_{ij}$] Series impedance of branch $(i,j)$
	\item[$\mathbf{Y}_{ij} = \mathbf{Z}^{-1}_{ij}$] Series admittance of branch $(i,j)$
	\item[$\mathbf{Y}^{sh}_{ij},\mathbf{Y}^{sh}_{ji}$] $\pi$-section shunt adm. of branch $(i,j)$
	\item[$\mathbf{Y}^{s}_{k}$] impedance of bus shunt element $k$
	\item[$\mathbf{S}_{k}^d := {[S^d_{k,c}]_{\phi \in \Phi}}$] Apparent power demand of load $k$
	\item[$\mathbf{S}_{ij}$] Apparent power flow of branch $(i,j)$
	\item[$\mathbf{S}_{k}^g := {[S^g_{k,c}]_{\phi \in \Phi}}$] Apparent power injection of generator $k$
\end{IEEEdescription} 
The notation $\mathbf{y} := \left[ y_c \right]_{\phi \in \Phi}$ indicates that the generic vector $\mathbf{y}$ collects the values of variable $y$ for all the cable conductors. 

Let $|\condsm|$ be the number of conductors. The apparent power flow $\mathbf{S}^{ij}$ and all the impedances are complex matrices $\mathbf{M}\in \mathbb{C}^{|\condsm| \times |\condsm|}$. No assumptions are made on the matrices, which can in general be asymmetrical. Notation $(\cdot)^H$ indicates the conjugate transpose of a matrix and $\text{diag}(\cdot)$ indicates the matrix's diagonal. 

\begin{figure}[h!]
  \includegraphics[width=\linewidth]{figures/draft_linemodel_limited_notation2.pdf}
  \caption{$\Pi$-model of a three-phase line as used in the present work. No assumption is made on $\mathbf{Z}_{ij},\mathbf{Y}^{sh}_{ij},\mathbf{Y}^{sh}_{ji}$: they can be asymmetrical and non-diagonal. }
  \label{fig:line}
\end{figure}

